The Age of Information in Multihop Networks

Information updates in multihop networks such as Internet of Things (IoT) and intelligent transportation systems have received significant recent attention. In this paper, we minimize the age of a single information flow in interference-free multihop networks. When preemption is allowed and the packet transmission times are exponentially distributed, we prove that a preemptive Last-Generated, First-Served (LGFS) policy results in smaller age processes across all nodes in the network than any other causal policy (in a stochastic ordering sense). In addition, for the class of New-Better-than-Used (NBU) distributions, we show that the non-preemptive LGFS policy is within a constant age gap from the optimum average age. In contrast, our numerical result shows that the preemptive LGFS policy can be very far from the optimum for some NBU transmission time distributions. Finally, when preemption is prohibited and the packet transmission times are arbitrarily distributed, the non-preemptive LGFS policy is shown to minimize the age processes across all nodes in the network among all work-conserving policies (again in a stochastic ordering sense). Interestingly, these results hold under quite general conditions, including (i) arbitrary packet generation and arrival times, and (ii) for minimizing both the age processes in stochastic ordering and any non-decreasing functional of the age processes.

==> sections/NWU.tex <==
\section{NWU Service Time Distribution}
In this section, we consider a more general service time distribution, which is New-Worse than Used (NWU) service time distribution. We also consider  in order arrival packets. In this case, the optimal policy is preemptive LGFS (policy $P$) (since the arrivals are in order, LCFS policy and LGFS policy have the same age performance), which is depicted in Algorithm \ref{alg1}. We next show that the preemptive LGFS policy is age-optimal in case of NWU service time distribution. 
\begin{theorem}\label{thmNWU}
If the packet service times are NWU and \emph{i.i.d.} across time and servers, then for all packet generation and arrival time sequence $a_1, a_2, \ldots$, where $a_1\leq a_2\leq \ldots$,  and all queue sizes $B$, the preemptive LGFS policy is age-optimal.
\end{theorem}

To prove Theorem \ref{thmNWU}, we need to define the completion time of a packet as following:
Define $c_{i,\pi}$ as the completion time of the packet with time stamp $s_i$ under policy $\pi$. Without loss of generality, let $y_l$ and $y_k$ denote the packets with time stamps $s_l$ and $s_k$, respectively, where $s_k\geq s_l$. If the packet $y_l$ is preempted by the packet $y_k$ or the packet $y_k$ is delivered while the packet $y_l$ is being processed, then we have 
\begin{equation*}
c_{l,\pi}=c_{k,\pi}.
\end{equation*}  

The key step in the proof of Theorem \ref{thmNWU} is the following lemma, where we compare policy $P$ with any work-conserving policy $\pi \in \Pi_{wc}$.

\begin{lemma}\label{lemNWU1}
suppose that, for a given time instant $t \in [0, \infty)$, there exist $n$ packets arrived to the system. Then, for any given sequence of time stamps $(s_1, \ldots, s_n)$ of the arrived packets, where $s_1\leq \ldots\leq s_n$, we have
\begin{equation}\label{lawNWU_1}
c_{i,P}\leq_{\text{st}} c_{i,\pi},  \quad \forall i=1,\ldots,n,
\end{equation}
for all $\pi\in\Pi_{wc}$.
\end{lemma}

\begin{proof}
See Appendix~\ref{Appendix_F}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thmNWU}]
Since the age is an increasing function of the packets completion time. As a result, Lemma \ref{lemNWU1} implies
\begin{equation}
\begin{split}
\{\Delta_{P}(t), t\in[0,\infty)\}\!\!\leq_{\text{st}} \!\!\{\Delta_{\pi}(t), t\in[0,\infty)\},~ \forall \pi\in\Pi_{wc}.\nonumber
 \end{split}
\end{equation}
Finally, since the service times are \emph{i.i.d.} across time and servers, service idling only increases the waiting time of the packet in the system. Therefore, the age under non-work-conserving policies will be greater. As a result, we have 
\begin{equation}
\begin{split}
 \!\!\!\!\!\!\!\{\Delta_{P}(t),  t\in[0,\infty)\}\leq_{\text{st}} \{\Delta_{\pi}(t), t\in[0,\infty)\}, \forall \pi\in\Pi.\nonumber
 \end{split}
\end{equation}
This completes the proof.
\end{proof}






%The proof of this Theorem is similar to the proof of Theorem \ref{thm1}. The proof idea is that, the preemptive LGFS policy starts serving the freshest packet before any other policy. The proof details are provided in Appendix~\ref{Appendix_F}.


==> sections/near_age_optimality.tex <==
\section{Near Age-optimality Results}\label{nao}

\begin{figure}
\includegraphics[scale=0.6]{figure/sys_model2.eps}
\centering
\caption{ Information updates over a multihop network, where each node in the network (except the gateway) is restricted to receive data from only one node.}\label{Fig:sysMod2}
\vspace{-0.3cm}
\end{figure}

While the policy space being considered in Theorem \ref{thm1} (for exponential transmission distributions) is very general, the policy space considered in Theorem \ref{thm2} (for general transmission distributions) is restricted to only non-preemptive work-conserving policies. The next question we answer is whether for an important class of distributions that are more general than exponential, optimality or near-optimality can be achieved without restricting to the class of non-preemptive work-conserving policies. 
%We consider the class of all causal policies $\Pi$.
 We propose a non-preemptive LGFS policy and show that it is within a small age gap of the optimum average age among all policies in $\Pi$. Notice that the non-prmp-LGFS policy is a causal policy, i.e., its scheduling
decisions are made based on the history and current information of the system and do not require the knowledge
of the future packet generation and arrival times. Although the generalization in the policy space and transmission time distributions, we are able to prove this result for a somewhat more restrictive network than the general topology  $\mathcal{G(V, L)}$. The network here is represented by a directed graph $\mathcal{G'}(\mathcal{V},\mathcal{L})$, in which each node $j\in \mathcal{V}\backslash \{0\}$ is allowed to receive data from only one node (the total number of incoming links to each node $j\in \mathcal{V}\backslash \{0\}$ is at most one), as shown in Fig. \ref{Fig:sysMod2}. 
 %Each link in the network maintains a queue with infinite buffer size, i.e., $B_{ij}=\infty$ for all $(i,j)\in \mathcal{L}$. 
 The packet transmission times are assumed to be \emph{i.i.d.} across time and links. We consider the classes of New-Better-than-Used (NBU) packet transmission time distributions, which are defined as follows.
\begin{definition}  \textbf{New-Better-than-Used distributions \cite{shaked2007stochastic}:} Consider a non-negative random variable $X$ with complementary cumulative distribution function (CCDF) $\bar{F}(x)=\mathbb{P}[X>x]$. Then, $X$ is \textbf{New-Better-than-Used (NBU)} if for all $t,\tau\geq0$
\begin{equation}\label{NBU_Inequality}
\bar{F}(\tau +t)\leq \bar{F}(\tau)\bar{F}(t).
\end{equation} 
\end{definition}
%In practice, NBU distributions include constant transmission time, (shifted) exponential distribution, geometrical distribution, Erlang distribution, etc. 
Examples of NBU \footnote{The word \textbf{better} in the terminology \textbf{New-Better-than-Used} refers to that a random variable with a long lifetime is better than that with a shorter lifetime. In our case, the random variable is the transmission time, and longer transmission time is worse in terms of the age. Thus, the word \textbf{better} here doesn't imply an improvement in the age performance.} distributions include constant transmission time, (shifted) exponential distribution, geometric distribution, Erlang distribution, negative binomial distribution, etc.

%Define a set of parameters $\mathcal{I}'=\{n,(s_i, a_{i0})_{i=1}^{n}, \mathcal{G'(V, L)}\}$
Define a set of the parameters $\mathcal{I}'=\{\mathcal{G'}(\mathcal{V}, \mathcal{L}), (B_{ij}, (i,j)\in\mathcal{L}),$  $s_l, a_{l0},l=1,2,\ldots\}$, where  $\mathcal{G'}(\mathcal{V}, \mathcal{L})$ is the network graph with the new restriction, $B_{ij}$ is the queue buffer size of the link $(i,j)$, $s_l$ is the generation time of packet $l$, and $a_{l0}$ is the arrival time of packet $l$ to node $0$. Define $\mathcal{H}_k$ as the set of nodes in the $k$-th hop, i.e., $\mathcal{H}_k$ is the set of nodes that are separated by $k$ links from node $0$ \footnote{Node $0$ is always considered to be in $\mathcal{H}_0$.}. Let $v_{lj}(\pi)$ denote the transmission starting time of packet $l$ over the incoming link to node $j$ under policy $\pi$. To show that policy non-prmp-LGFS can come close to age-optimal, we need to construct an age lower bound. We will construct an infeasible policy which provides the age lower bound as follows:
\begin{itemize}
\item The infeasible policy ($IP$) is constructed as follows. At each link $(i,j)$, the packets are served by following a work-conserving LGFS principle. A packet $l$ is deemed delivered from node $i$ to node $j$ once the transmission of packet $l$ starts over the link $(i,j)$ (this step is infeasible). After the transmission of packet $l$ starts over the link $(i,j)$, the link $(i,j)$ will be busy for a time duration equal to the actual transmission time of packet $l$ over the link $(i,j)$. Hence, the next packet cannot start its transmission over the link $(i,j)$ until the end of this time duration. We use $v_{lj}(IP)$ to denote the transmission starting time of packet $l$ over the incoming link to node $j$ under the infeasible policy ($IP$) constructed above.

 \begin{figure}[!tbp]
 \centering
 \subfigure[Two-hop tandem network.]{
  \includegraphics[scale=0.9]{figure/3_hops_NW.eps}
   \label{f_a}
   }
 \subfigure[A sample path of the packet arrival processes.]{
  \includegraphics[scale=0.36]{figure/lowerbound_illu.eps}
   \label{f_b}
   }
\caption{An illustration of the infeasible policy in a Two-hop network.} \label{fig:arrival_sample_1}
\end{figure}
One example of the infeasible policy IP is illustrated in Fig. \ref{fig:arrival_sample_1}, where we consider two hops of tandem queues. We use $t^l_j$ to denote the time by which the incoming link to node $j$ becomes idle again after the transmission of packet $l$ starts.  Since all links are idle at the beginning, packet 1 arrives to all nodes once it arrives to node 0 at time $a_{10}$ (this is because each packet is deemed delivered to the next node once its transmission starts). However, each link is kept busy for a time duration equal to the actual transmission time of packet 1 over each link. Then, packet 2 arrives to node 0 at time $a_{20}$ and finds the link $(0,1)$ busy. Therefore, packet 2 cannot start its transmission until link $(0,1)$ becomes idle again at time $t^1_1$ $(v_{21}(IP)=t^1_1)$. Once packet 2 starts its transmission at time $t^1_1$ over the link $(0,1)$, it is deemed delivered to node 1 $(a_{21}(IP)=v_{21}(IP)=t^1_1)$ and link $(0,1)$ is kept busy until time $t^2_1$. At time $t^1_1$, link $(1,2)$ is busy. Thus, packet 2 cannot start its transmission over the link $(1,2)$ until it becomes idle again at time $t^1_2$. Once packet 2 starts its transmission over the link $(1,2)$ at time $t^1_2$, it is deemed delivered to node 2 $(a_{22}(IP)=v_{22}(IP)=t^1_2)$.

%The same operation is repeated at links $(1,2)$ and $(2,3)$, where packet 2 waits in the queue of the link $(1,2)$ until it becomes idle again at time $t^1_2$, then, it is considered delivered to node 2 at time $(a_{22}(IP)=v_{22}(IP)=t^1_2)$ and link $(1,2)$ is kept busy in sending a virtual copy of packet 2 until time $t^2_2$. Finally, packet 2 arrives to the link $(2,3)$ and finds it idle. Thus, packet 2 is delivered immediately to node 3 once it arrives to the link $(2,3)$ $(a_{23}(IP)=v_{23}(IP)=a_{22}(IP))$, and the link $(2,3)$ is kept busy in sending a virtual copy of packet 2 until time $t^2_3$.}

\item The age lower bound is constructed as follows. For each node $j\in\mathcal{V}$, define a function $\Delta_{j,IP}^{\text{LB}}(t)$ as
\begin{equation}\label{lower_bound_def_1}
\Delta_{j,IP}^{\text{LB}}(t)=t-\max\{s_l : v_{lj}(IP)\leq t\}.
\end{equation}
The definition of the $\Delta_{j,IP}^{\text{LB}}(t)$ is similar to that of the age in \eqref{age} except that the packets arrival times to node $j$ are replaced by their transmission starting times over the incoming link to node $j$ in the infeasible policy. In this case, $\Delta_{j,IP}^{\text{LB}}(t)$ increases linearly with $t$ but is reset to a smaller value with the transmission start of a fresher packet over the incoming link to node $j$, as shown in Fig. \ref{Fig:age_lower_at_node_one}. The process of $\Delta_{j,IP}^{\text{LB}}(t)$ is given by $\Delta_{j,IP}^{\text{LB}}=\{\Delta_{j,IP}^{\text{LB}}(t), t\in [0,\infty)\}$ for each $j\in\mathcal{V}$. The age lower bound vector of all the network nodes is 
\begin{align}
\mathbf{\Delta}^{\text{LB}}_{IP}(t)=\!\!(\Delta_{0,IP}^{\text{LB}}(t), \Delta_{1,IP}^{\text{LB}}(t), \ldots, \Delta_{N-1,IP}^{\text{LB}}(t)). 
\end{align}
The age lower bound process of all the network nodes is given by
\begin{align}
\mathbf{\Delta}_{IP}^{\text{LB}}=\{\mathbf{\Delta}^{\text{LB}}_{IP}(t), t\in [0,\infty)\}.
\end{align}
\begin{figure}
\centering \includegraphics[scale=0.38]{figure/lower_bound_graph.eps}
\centering
\captionsetup{justification=justified, font={small,onehalfspacing}}
\caption{The evolution of $\Delta_{j,IP}^{\text{LB}}(t)$ and $\Delta_{j,\pi}(t)$ at node $j\in\mathcal{H}_1$. For figure clarity, we use $v_1$ and $v_2$ to denote $v_{1j}(IP)$ and $v_{2j}(IP)$, respectively. Also, we use $a_1$ and $a_2$ to denote $a_{1j}(\pi)$ and $a_{2j}(\pi)$, respectively. We suppose that $a_{10}>s_1$ and $a_{20}>a_1>s_2$, such that $a_{10}=v_1$ and $a_{20}=v_2$. }\label{Fig:age_lower_at_node_one}
\vspace{-0.3cm}
\end{figure}
\end{itemize}
%Hop 0: Since the packet arrival times $(a_{10}, a_{20}, \ldots, a_{n0})$ at node $0$ are invariant of the scheduling policy $\pi$, the age at node 0 is invariant of the scheduling policy too. Hence, we define a function $\Delta_{0,\pi}^{\text{LB}}(t)=\Delta_{0,\pi}(t)$.}  
%
%\item \textcolor[rgb]{0.00,0.00,1.00}{Hop 1: For each node $j\in\mathcal{H}_1$, define a function $\Delta_{j,\pi}^{\text{LB}}(t)$ as
%\begin{equation}\label{lower_bound_def_1}
%\Delta_{j,\pi}^{\text{LB}}(t)=t-\max\{s_l : v_{lj}(\pi)\leq t\}.
%\end{equation}
%The definition of the $\Delta_{j,\pi}^{\text{LB}}(t)$ is similar to that of the age of policy $\pi$ at node $j$ except that the packets arrival times to node $j$ are replaced by their transmission starting times at the link $(0,j)$. In this case, $\Delta_{j,\pi}^{\text{LB}}(t)$ increases linearly with $t$ but is reset to a smaller value with the transmission start of a fresher packet over the link $(0,j)$, as shown in Fig. \ref{Fig:age_lower_at_node_one}.} 
%%Thus, the packets are considered to be delivered to node $j$ at time $(v_{1j}(\pi), \ldots, v_{nj}(\pi))$. 
% 
% \begin{figure}[!tbp]
% \centering
% \subfigure[Three hops tandem network.]{
%  \includegraphics[scale=0.9]{figure/3_hops_NW.eps}
%   \label{f_a}
%   }
% \subfigure[A sample path of the packet arrival processes.]{
%  \includegraphics[scale=0.4]{figure/lowerbound_illu.eps}
%   \label{f_b}
%   }
%\caption{An illustration of the age lower bound in a three-hop network.} \label{fig:arrival_sample_1}
%\end{figure}
%\item \textcolor[rgb]{0.00,0.00,1.00}{Hop $k\geq 2$: For the nodes in the subsequent hops (the nodes in $\mathcal{H}_k$ such that $k\geq 2$), the lower bound acts as an infeasible policy separately from policy $\pi$. The policy LB (the infeasible policy) is constructed as follows. The packets at each link queue are served in LGFS manner. Each packet $l$ is considered to be delivered from node $i$ to node $j$ once the transmission of packet $l$ starts over the link $(i,j)$; however,  after the transmission of packet $l$ starts over the link $(i,j)$, the link $(i,j)$ becomes busy in sending a virtual copy of packet $l$ for a duration equal to the transmission time of packet $l$ at the link $(i,j)$.}
%
%
% 
% 
% 
% From this, we conclude that  $a_{lj}(\text{LB})=v_{lj}(\text{LB})$ for all $l=1,\ldots, n$ and all $j\in\mathcal{H}_k$ such that $k\geq 2$. The function $\Delta_{j,\pi}^{\text{LB}}(t)$ is defined at each node $j\in\mathcal{H}_k$ for $k\geq 2$ as 
%\begin{equation}\label{lower_bound_def_2}
%\Delta_{j,\pi}^{\text{LB}}(t)=t-\max\{s_l : v_{lj}(\text{LB})\leq t\}.
%\end{equation}

The next Lemma tells us that the process $\mathbf{\Delta}_{IP}^{\text{LB}}$ is an age lower bound of all policies in $\Pi$ in the following sense. 
\begin{lemma}\label{lem_lower_bound_all}
Suppose that the packet transmission times are NBU and \emph{i.i.d.} across time and links, then for all $\mathcal{I}'$ satisfying $B_{ij}\geq 1$ for each $(i,j)\in\mathcal{L}$, and $\pi\in\Pi$
\begin{align}\label{lower_bound_equation}
[\mathbf{\Delta}^{\text{LB}}_{IP}\vert\mathcal{I}']\leq_{\text{st}} [\mathbf{\Delta_{\pi}}\vert\mathcal{I}'].
\end{align}
%[\Delta_{j,\text{non-prmp-LGFS}}^{\text{LB}}\vert\mathcal{I}']\leq_{\text{st}} [\Delta_{j,\pi},\vert\mathcal{I}],~\forall j\in\mathcal{V}
%\begin{equation}\label{hypo_na1}
%[\mathbf{\Gamma}_j(VP)\vert\mathcal{I}']\leq_{\text{st}} [\mathbf{D}_j(\pi)\vert\mathcal{I}'],\quad\forall j\in\mathcal{V},
%\end{equation}
%or equivalently, for all $\mathcal{I}'$ and $\pi\in\Pi_{np}$
%\begin{equation}\label{hypo_na2}
%[\{\Delta_{j,VP}(t), t\in [0,\infty)\}\vert\mathcal{I}']\leq_{\text{st}} [\{\Delta_{j,\pi}(t), t\in [0,\infty)\}\vert\mathcal{I}'],
%\end{equation}
%holds for all $j\in\mathcal{V}$.
\end{lemma}
\begin{proof}
See Appendix~\ref{Appendix_C}.
\end{proof}

We can now proceed to characterize the age performance of policy non-prmp-LGFS among policies in $\Pi$. Let $X_{ij}$ denote the packet transmission time over the link $(i,j)$, with mean $\mathbb{E}[X_{ij}]=\mathbb{E}[X]<\infty$ for all $(i,j)\in \mathcal{L}$. We use Lemma \ref{lem_lower_bound_all} to prove the following theorem. 
%Then, the age performance of non-preemptive LGFS policy among the policies in $\Pi$ is characterized in the following theorem.
\begin{theorem}\label{thmnbu_gab}
Suppose that the packet transmission times are NBU and \emph{i.i.d.} across time and links, then for all $\mathcal{I}'$ satisfying $B_{ij}\geq 1$ for each $(i,j)\in\mathcal{L}$
\begin{equation}\label{gap_main1}
\begin{split}
&\min_{\pi\in\Pi}[\bar{\Delta}_{j,\pi}\vert\mathcal{I}']\leq [\bar{\Delta}_{j, \text{non-prmp-LGFS}}\vert\mathcal{I}']\leq\\&
\min_{\pi\in\Pi}[\bar{\Delta}_{j,\pi}\vert\mathcal{I}'] + (2k-1)\mathbb{E}[X],~\forall j\in\mathcal{H}_k, \forall k\geq 1,
\end{split}
\end{equation}
where $\bar{\Delta}_{j,\pi}=\limsup_{T\rightarrow\infty}\frac{\mathbb{E}[\int_{0}^{T}\Delta_{j,\pi}(t)dt]}{T}$ is the average age at node $j$ under policy $\pi$.
\end{theorem}
\begin{proof}
See Appendix~\ref{Appendix_D}.
\end{proof}
Theorem \ref{thmnbu_gab} tells us that for arbitrary sequence of packet generation times $\{s_1, s_2, \ldots\}$, sequence of arrival times $\{a_{10}, a_{20}, \ldots\}$ at node $0$, and buffer sizes $(B_{ij}\geq 1,(i,j)\in\mathcal{L})$, the non-prmp-LGFS policy is within a constant age gap from the optimum average age among all policies in $\Pi$. 

It is worth observing that the results in Theorem \ref{thm1}, Theorem \ref{thm2}, and Theorem \ref{thmnbu_gab} hold for any link buffer sizes $B_{ij}$'s. Hence, the buffer sizes can be chosen according to the application. In particular, in some applications, such as  news and social updates, users are interested in not just the latest updates, but also past news. Thus, in such application, we may need to have queues with buffer sizes greater than one to store old packets and send them later whenever links become idle. On the other hand, there are some other applications, in which old packets become useless when the fresher packets exist. Thus, in these applications, buffer sizes can be chosen to be zero (one) when we follow the prmp-LGFS (non-prmp-LGFS) scheduling policy. 
\subsection{Simulation Results}
%\begin{figure}
%\includegraphics[scale=0.6]{figure/Sim2_network.eps}
%\centering
%\caption{ A  multihop network.}\label{Fig:simulation2}
%\vspace{-0.3cm}
%\end{figure}
We now provide a simulation result to illustrate the age performance of different policies when the transmission times are NBU. We consider the network in Fig. \ref{Fig:sysMod2}. 
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/Avg_age_kchange_A_30_s_2_10.eps}
\caption{Average age at node 5 under gamma transmission time distributions at each link with different shape parameter $\beta$.}
\vspace{-.0in}
\label{avg_age3}
\end{figure}
Figure \ref{avg_age3} illustrates the average age at node 5 under gamma transmission time distributions at each link with different shape parameter $\beta$, where the buffer sizes are either 1, 10, or 100. The mean of the gamma transmission time distributions at each link is normalized to 0.2. The inter-generation times are \emph{i.i.d.} Erlang-2 distribution with mean $1/\lambda=1/30$. The time difference ($a_{i0}-s_i$) between packet generation and arrival to node $0$ is Zero. Note that the average age of the FCFS policy with infinite buffer sizes is extremely high in this case and hence is not plotted in this figure. The ``Age lower bound'' curve is generated by using $\frac{\int_{0}^{T}\Delta_{5,IP}^{LB}}{T}$ when the buffer sizes are 1 which, according to Lemma \ref{lem_lower_bound_all}, is a lower bound of the optimum average age at node 5. We can observe that the gap between the ``Age lower bound'' curve and the average age of the non-prmp-LGFS policy at node 5 is no larger than $9E[X] = 1.8$, which agrees with Theorem \ref{thmnbu_gab}. In addition, we can observe that prmp-LGFS policy achieves the best age performance among all
plotted policies when $\beta=1$. This is because a gamma distribution with shape parameter $\beta=1$ is an exponential distribution. Thus, age-optimality can be achieved in this case by policy prmp-LGFS as stated in Theorem \ref{thm1}. However, as can be seen in the figure, the average age at node 5 of the prmp-LGFS policy blows up as the shape parameter $\beta$ increases and the non-prmp-LGFS policy achieves the best age performance among all plotted policies when $\beta>2$. The reason for this phenomenon is as follows: As $\beta$ increases, the variance (variability) of normalized gamma distribution decreases. Hence, when a packet is preempted, the service time of a new packet is probably longer than the remaining service time of the preempted packet. Because the generation rate is high, packet preemption happens frequently, which leads to infrequent packet delivery and increases the age. This phenomenon occurs heavily at the first link (link $(0,1)$) which, in turn, affects the age at the subsequent nodes. 






%Define $W_{ij}=a_{ij}-s_i$. The following corollary is a consequence of Theorem \ref{thmnbu_gab}.
%\begin{corollary}\label{cornbu_gab}
%Suppose that the packet transmission times are NBU and \emph{i.i.d.} across time and links, and $\mathbb{E}[W^2_{ij}]<\infty$ for all $i=\{1, \ldots, n\}$ and $j\in\mathcal{V}$, then for all $\mathcal{I}$ satisfying $B_{ij}\geq 1$ for each $(i,j)\in\mathcal{L}$
%\begin{align*}
%\min_{\pi\in\Pi} \mathbf{\bar{\Delta}}_{\pi}\leq \mathbf{\bar{\Delta}}_{\text{non-prmp-LGFS}}\leq 3\min_{\pi\in\Pi} \mathbf{\bar{\Delta}}_{\pi}, 
%\end{align*}
%where $\mathbf{\bar{\Delta}}_\pi=\left(\bar{\Delta}_{0,\pi}, \bar{\Delta}_{1,\pi}, \ldots, \bar{\Delta}_{N-1,\pi}\right)$.
%\end{corollary}
%
%\begin{proof}



%We provide a proof sketch of Theorem \ref{thm3}. We will prove this theorem in three steps: in \emph{Step 1}, we will construct a virtual policy which provides an age lower bound of $\{\Delta_j(t), t\in [0,\infty)\}$ at each node $j\in\mathcal{V}$; in \emph{Step 2}, we prove that the constructed virtual policy is age optimal at each node of the network among the policies in $\Pi_{np}$; in \emph{Step 3}, we will evaluate the age gap between the age lower bound and the average age of non-preemptive LGFS policy. 
%\ifreport
%See Appendix~\ref{Appendix_E}.
%\end{proof}

%
%\begin{align*}
%\min_{\pi\in\Pi_{np}} \bar{\Delta}_{j,\pi}\leq \bar{\Delta}_{j, \text{non-prmp-LGFS}}\leq\min_{\pi\in\Pi_{np}} \bar{\Delta}_{j,\pi} + (2k-1)\mathbb{E}(X), 
%\end{align*}
%or equivalently, ,

%In this section, we focus on the network consisting of $N$ nodes, where  We represent this network by a directed graph $\mathcal{G'}(\mathcal{V},\mathcal{L})$, where $\mathcal{V}$ is the set of nodes and $\mathcal{L}$ is the set of links. Let $H_k$ denote the set of nodes in the $k$-th hop (that are separated by $k$ links from node $0$), where node $0$ is always considered to be in $H_0$.

%We define the competitive ratio of a policy $\beta$ as the maximum ratio of the achieved average age of all nodes in the network for policy $\beta$ to the achieved average age of all nodes in the network for an optimal virtual policy.
